The connected Grundy coloring problem: Formulations and a local-search enhanced biased random-key genetic algorithm

Given a graph G=(V,E), a connected Grundy coloring is a proper vertex coloring that can be obtained by a first-fit heuristic on a connected vertex sequence. A first-fit coloring heuristic is one that attributes to each vertex in a sequence the lowest-index color not used for its preceding neighbors. A connected vertex sequence is one in which each element, except for the first one, is connected to at least one element preceding it. The connected Grundy coloring problem consists of obtaining a connected Grundy coloring maximizing the number of colors. In this paper, we propose two integer programming (IP) formulations and a local-search enhanced biased random-key genetic algorithm (BRKGA) for the connected Grundy coloring problem. The first formulation follows the standard way of partitioning the vertices into color classes while the second one relies on the idea of representatives in an attempt to break symmetries. The BRKGA encompasses a local search procedure using a newly proposed neighborhood. A theoretical neighborhood analysis is also presented. Extensive computational experiments indicate that the problem is computationally demanding for the proposed IP formulations. Nonetheless, the formulation by representatives outperforms the standard one for the considered benchmark instances. Additionally, our BRKGA can find high-quality solutions in low computational times for considerably large instances, showing improved performance when enhanced with local search and a reset mechanism. Moreover we show that our BRKGA can be easily extended to successfully tackle the Grundy coloring problem, i.e., the one without the connectivity requirements.

==> 70_greedycolorings.tex <==
\section{Classical greedy coloring heuristics}
\label{sec:classicalgreedycoloring}

In this section, we detail four well-known and widely-used greedy criteria for first-fit heuristics to obtain a proper coloring of a graph. Namely, we present the criteria: maximum-degree first, adaptive maximum-degree first, smallest-degree last, and maximum saturation degree first (DSatur). We emphasize that our goal is to present the idea of the order determined by these criteria, and not to analyze running times and implementation details of the involved algorithms.

Consider a graph $G=(V,E)$ and a set of available colors $K = \{1,\ldots,\Delta(G)+1$\}.
In what follows, each of the presented greedy criteria defines a sequence (ordering) $(v_1,\ldots,v_n)$ of the vertices in $V$. It is assumed that each vertex in the order will receive the lowest possible color. Define the \textit{saturation degree} of a vertex as the number of different colors adjacent to it, i.e., the number of different colors assigned to its neighbors.

\begin{enumerate}

\item The \textit{maximum-degree first} criterion establishes that the sequence $(v_1,\ldots,v_n)$ is given by the vertices in $V$ in nonincreasing order of their degrees.
\item The \textit{adaptive-maximum degree first} criterion defines a sequence $(v_1,\ldots,v_n)$ as detailed in Algorithm~\ref{alg:adaptivemaxdegree}.
\begin{algorithm}[!ht]
\caption {Adaptive maximum-degree first ($G$)}
\label{alg:adaptivemaxdegree}
    $H \leftarrow G$\;
    \ForEach{$j=1$ to $n$}{
        $v_j \leftarrow$ vertex $u$ with maximum degree in $H$\;
        $H \leftarrow H - v_{j}$\;
    }
    \Return the sequence $(v_1,v_2,\ldots,v_n)$\; 
\end{algorithm}
\item The \textit{smallest-degree last} criterion~\cite{MatBec83} builds a sequence $(v_1,\ldots,v_n)$ as presented in Algorithm~\ref{alg:smallestdegree}.
\begin{algorithm}[!ht]
\caption {Smallest-degree last ($G$)}
\label{alg:smallestdegree}
    $H \leftarrow G$\;
    \ForEach{$j=n$ down to $1$}{
        $v_j \leftarrow$ vertex $u$ with minimum degree in $H$\;
        $H \leftarrow H - v_{j}$\;
    }
    \Return the sequence $(v_1,v_2,\ldots,v_n)$\; 
\end{algorithm}
\item \textit{DSatur}~\cite{Bre79} constructs a sequence $(v_1,\ldots,v_n)$ using an adaptive criterion based on the maximum saturation degree as described in Algorithm~\ref{alg:dsatur}.
\begin{algorithm}[!ht]
\caption {DSatur ($G$)}
\label{alg:dsatur}
    $H \leftarrow G$\;
    $v_1 \leftarrow$ vertex of maximum degree in $H$\;
    $H \leftarrow H - v_{1}$\;
    \ForEach{$j=2$ to $n$}{
        $v_j \leftarrow$ vertex $u \in V(H)$ with maximum saturation degree in $G$ or, in case of ties, the vertex $u$ with maximum degree in $H$\;
        $H \leftarrow H - v_{j}$\;
    }
    \Return the sequence $(v_1,v_2,\ldots,v_n)$\;
\end{algorithm}

\end{enumerate}

\newpage
Notice that, differently from the other criteria presented in this section, DSatur always results in a connected coloring.




==> 90_somenotes.tex <==





\rafaelF{Ainda não sei o objetivo final do lema que segue, mas ele não está relacionado à vizinhança sendo analisada.}\MateusF{Esse foi um dos que eu tinha listado quando estava tentando descobrir o que seria útil. Terminamos não usando, assim como aquele que era o caso do vértice que pode ser removido sem alterar nada}\MateusF{Se não me engano, foi quando a gente estava considerando fazer um swap de dois vértices, ao invés do move, mas era bem mais demorado e tinha mudanças mais drásticas}
\begin{lemma}
\label{lemma:gemini}
\rafaelC{Consider a solution $S$ and two vertices $v$ and $u$ such that $p_{S}(v) = i$, $p_{S}(u) = j$, and $N(v)-\{u\} = N(u)-\{v\}$. The solution $S'$ obtained from $S$ by swapping the positions of $u$ and $v$ results into the same connected Grundy coloring as $S$ except for the colors of $v$ and $u$, that are swapped.}
\end{lemma}
\begin{proof}
\rafaelC{The proof follows directly. Let $S'$ be the sequence obtained by swapping the positions of $v$ and $u$ in $S$ and assume without loss of generality that $i \leq j$. Observe that $S$ and $S'$ lead to the same color to all the vertices before position $i$. Furthermore, $c_{S'}(u) = c_{S}(v)$ as they have the same neighborhood and all the vertices in the interval $[i+1, \ldots, j-1]$ receive the same color in $c_S$ and $c_{S'}$ due to the same fact. Finally, notice that $c_{S'}(v) = c_{S}(u)$, because the colors determined by $c_S$ and $c_{S'}$ are the same upon that point and then all the remaining vertices receive the same color in both colorings. }
\end{proof}


\rafaelF{Parei aqui.}
\rafaelF{O lema abaixo está relacionado à vizinhança?}
\MateusF{Mais ou menos kkkk esse é o que Márcio generalizou do que eu estava fazendo em relação a aresta de corte. O objetivo era mostrar que sobre certas condições as colorações dos subgrafos eram idependentes. Nesse sentido existem muitos moves que não alteram a coloração. E seria um pouco da premissa para o método de conexão das instâncias}

\marcioC{
\begin{lemma}
\label{lemma:cut}
Given a connected sequence $\sigma_c$ and a cut $C \subseteq E(G)$, then every connected sequence $\sigma_c^{*}$ that agrees with $\sigma_c$ in relation to $V(C)$ and in relation to $V(H_i)$, where $H_i$ are the connected components obtained from $G$ by the removal of $C$, produces that same greedy connected coloring. 
\end{lemma}
\begin{proof}
By absurdity, consider two connected sequences $\sigma_c$ and $\sigma_c^{*}$ that agree in relation to $V(C)$ and in relation to $V(H_i)$, but produce two different colorings $c$ and $c^*$. Let $v$ be the first vertex according to
$\sigma_c$ that has a color in $c$ different from the one assigned in $c^*$. Notice that for $c(v) \not= c^{*}(v)$ we must have either a different set of neighbors that appears before $v$ in $\sigma_c$ and $\sigma_c^{*}$ or the set of colors assigned to the neighbors is different.\\
On the one hand, assume that the set of neighbors that appears before $v$ in $\sigma_c$ and in $\sigma_c^{*}$ are different. W.l.o.g. assume that we have a neighbor $u$ that comes before from $v$ in $\sigma_c$ but after in $\sigma_c^{*}$, as this vertex cannot be in the same connected component of $v$, because the connected sequences agree with each component, this vertex must belong to a different connect component, hence the edge $vu$ must be in the cut $C$, what is also impossible since the connected sequences must also agree with respect to $V(C)$.\\
On the other hand, as the set of neighbors that appear before $v$ in $\sigma_c$ and $\sigma_c^{*}$ are the same, then all must have received the same color, due to the choice of $v$. Then, $c(v) = c^{*}(v)$.
\end{proof}
}






\section{two-index formulation for connected Grundy?}


$z_{vt}$ if vertex $v$ is colored in time $t$.



\begin{flalign}
 \max & \sum_{k \in K} w_{k} & & \label{tgru:obj}\\
& x_{uk} + x_{vk} \leq 1, & {\rm \forall \ } k \in K, \ uv \in E, & \label{tgru:01} \\
& \sum_{k \in K} x_{vk} \leq 1, & {\rm \forall \ } v \in V, & \label{tgru:02} \\
& w_{k} \leq \sum_{v \in V} x_{vk} , & {\rm \forall \ } k \in K, & \label{tgru:03} \\
&  x_{vk'} \leq \sum_{u \in N(v)} x_{uk}, & {\rm \forall \ } v \in V, \ k,k' \in K, \textrm{ with } k < k', \label{tgru:04}\\
%&  w_{vk'} \leq \sum_{u \in N(v)} x_{uk}, & {\rm \forall \ } k,k' \in K, {\textrm with \ } k < k', \label{gru:05}\\
&  w_{k'} \leq w_{k}, & {\rm \forall \ } k,k' \in K, \textrm{ with } k < k', \label{tgru:06}\\
& x_{uk} \in \{0,1\}, & {\rm \forall \ } u \in V, \ k \in K, & \label{tgru:07} \\
& w_{k} \in \{0,1\}, & {\rm \forall \ } k \in K. & \label{tgru:08}\\
&  \sum_{t \in T} z_{vt} = 1 , & {\rm \forall \ } v \in V, \label{tgru:09}\\
&  \sum_{v \in V} z_{vt} = 1 , & {\rm \forall \ } t \in T, \label{tgru:10}
\end{flalign}



  
  
  

==> 92_appendice_brkga_novo.tex <==
\section{old results - BRKGA}


\begin{comment}
\begin{table}[ht]
\centering
\footnotesize
\captionsetup{font=small}
\caption{BRKGA results for the bipartite instances}
\begin{tabular}{l|rrr|rrrrr|rrrrr}
  \hline
\multicolumn{1}{c|}{} & 
\multicolumn{3}{c|}{BRKGA} & 
\multicolumn{5}{c|}{BRKGA+R} & 
\multicolumn{5}{c}{BRKGA+R+LS} \\
instance & mean & max & ttb & mean & max & ttb & $diff_{m}$ & $diff_{x}$ & mean & max & ttb & $diff_{m}$ & $diff_{x}$ \\ 
\hline
bip\_50\_0.2 &  7.6 &  8.0 &  31.2 &  7.8 &  8.0 &  72.6 & 3.0 & 0.0 &  7.8 &  8.0 &  70.3 & 3.2 & 0.0 \\ 
  bip\_50\_0.4 & 10.1 & 11.0 &  19.6 & 10.2 & 11.0 &  77.1 & 1.7 & 0.0 & 10.2 & 11.0 &  51.5 & 1.4 & 0.0 \\ 
  bip\_50\_0.6 & 12.8 & 13.4 &  65.1 & 13.0 & 13.8 &  95.9 & 2.1 & 3.1 & 13.0 & 13.8 &  78.9 & 1.9 & 3.1 \\ 
  bip\_50\_0.8 & 14.9 & 16.0 &  59.4 & 15.6 & 16.4 & 149.5 & 4.3 & 2.4 & 15.6 & 16.2 & 147.8 & 4.2 & 1.4 \\ 
  bip\_60\_0.2 &  8.2 &  8.6 &  19.4 &  8.5 &  9.0 & 104.3 & 4.8 & 5.0 &  8.5 &  9.0 &  95.9 & 4.5 & 5.0 \\ 
  bip\_60\_0.4 & 10.9 & 11.6 &  53.3 & 11.1 & 11.6 &  55.9 & 2.0 & 0.0 & 11.1 & 11.8 &  60.2 & 1.9 & 1.8 \\ 
  bip\_60\_0.6 & 13.9 & 15.0 &  82.5 & 14.2 & 15.0 & 138.9 & 2.2 & 0.0 & 14.2 & 15.0 & 119.7 & 2.2 & 2.7 \\ 
  bip\_60\_0.8 & 17.2 & 18.8 &  92.7 & 17.9 & 19.2 & 225.3 & 4.3 & 2.2 & 18.0 & 19.0 & 204.5 & 4.6 & 3.2 \\ 
  bip\_70\_0.2 &  8.6 &  9.2 &  27.7 &  9.0 &  9.2 & 105.0 & 4.1 & 0.0 &  9.0 &  9.2 &  94.6 & 3.9 & 0.0 \\ 
  bip\_70\_0.4 & 11.7 & 12.4 &  62.4 & 11.9 & 13.0 &  65.7 & 1.9 & 4.9 & 11.9 & 12.8 &  80.4 & 2.3 & 3.3 \\ 
  bip\_70\_0.6 & 14.6 & 15.8 &  81.9 & 15.1 & 16.0 & 165.0 & 3.0 & 1.2 & 15.1 & 16.0 & 162.5 & 3.0 & 1.3 \\ 
  bip\_70\_0.8 & 18.4 & 20.2 & 110.7 & 19.1 & 20.4 & 220.3 & 3.8 & 1.1 & 19.1 & 20.2 & 214.5 & 3.9 & 0.0 \\ 
  bip\_80\_0.2 &  9.4 &  9.8 &  49.1 &  9.8 &  9.8 &  71.2 & 4.6 & 0.0 &  9.8 &  9.8 &  81.8 & 4.4 & 0.0 \\ 
  bip\_80\_0.4 & 12.8 & 13.8 &  76.3 & 13.1 & 14.0 & 105.4 & 2.1 & 1.5 & 13.1 & 14.0 & 103.8 & 2.0 & 1.5 \\ 
  bip\_80\_0.6 & 16.0 & 17.0 & 108.6 & 16.4 & 17.8 & 178.8 & 2.8 & 4.7 & 16.4 & 17.4 & 174.6 & 2.5 & 2.4 \\ 
  bip\_80\_0.8 & 19.4 & 21.2 & 115.7 & 20.4 & 21.6 & 263.7 & 5.2 & 1.9 & 20.3 & 21.6 & 244.7 & 4.9 & 1.9 \\ 
   \hline
Mean & 12.9 & 13.8 & 65.9 & 13.3 & 14.1 & 130.9 & 3.2 & 1.7 & 13.3 & 14.0 & 124.1 & 3.1 & 1.7 \\
\hline
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\footnotesize
\captionsetup{font=small}
\caption{BRKGA results for the complement of bipartite instances}
\begin{tabular}{l|rrr|rrrrr|rrrrr}
  \hline
\multicolumn{1}{c|}{} & 
\multicolumn{3}{c|}{BRKGA} & 
\multicolumn{5}{c|}{BRKGA+R} & 
\multicolumn{5}{c}{BRKGA+R+LS} \\
instance & mean & max & ttb & mean & max & ttb & $diff_{m}$ & $diff_{x}$ & mean & max & ttb & $diff_{m}$ & $diff_{x}$ \\ 
  \hline
cbip\_50\_0.2 & 34.5 & 34.6 & 16.6 & 34.6 & 34.6 & 19.5 & 0.2 & 0.0 & 34.6 & 34.6 & 13.6 & 0.2 & 0.0 \\ 
  cbip\_50\_0.4 & 31.0 & 31.2 &  4.8 & 31.2 & 31.2 & 24.1 & 0.5 & 0.0 & 31.2 & 31.2 & 26.0 & 0.5 & 0.0 \\ 
  cbip\_50\_0.6 & 29.2 & 29.2 &  3.9 & 29.2 & 29.2 &  2.6 & 0.1 & 0.0 & 29.2 & 29.2 &  2.4 & 0.1 & 0.0 \\ 
  cbip\_50\_0.8 & 30.4 & 30.4 &  1.4 & 30.4 & 30.4 &  0.7 & 0.0 & 0.0 & 30.4 & 30.4 &  0.5 & 0.0 & 0.0 \\ 
  cbip\_60\_0.2 & 41.3 & 41.4 &  9.2 & 41.4 & 41.4 & 29.8 & 0.3 & 0.0 & 41.4 & 41.4 & 24.2 & 0.2 & 0.0 \\ 
  cbip\_60\_0.4 & 37.8 & 38.2 & 11.4 & 38.0 & 38.2 & 32.5 & 0.4 & 0.0 & 38.0 & 38.2 & 32.7 & 0.3 & 0.0 \\ 
  cbip\_60\_0.6 & 35.3 & 35.8 &  6.3 & 35.6 & 35.8 & 63.5 & 0.7 & 0.0 & 35.6 & 35.8 & 72.3 & 0.7 & 0.0 \\ 
  cbip\_60\_0.8 & 34.5 & 34.6 & 19.3 & 34.6 & 34.6 & 23.1 & 0.2 & 0.0 & 34.6 & 34.6 & 25.5 & 0.2 & 0.0 \\ 
  cbip\_70\_0.2 & 46.8 & 47.2 &  9.6 & 46.9 & 47.2 & 40.2 & 0.4 & 0.0 & 46.9 & 47.2 & 30.4 & 0.3 & 0.0 \\ 
  cbip\_70\_0.4 & 44.5 & 44.8 &  8.6 & 44.6 & 44.8 & 31.3 & 0.2 & 0.0 & 44.6 & 44.8 & 31.7 & 0.2 & 0.0 \\ 
  cbip\_70\_0.6 & 41.7 & 41.8 & 16.6 & 41.8 & 41.8 & 35.6 & 0.2 & 0.0 & 41.8 & 41.8 & 40.3 & 0.2 & 0.0 \\ 
  cbip\_70\_0.8 & 41.1 & 41.2 &  1.4 & 41.2 & 41.2 & 11.8 & 0.1 & 0.0 & 41.2 & 41.2 & 15.2 & 0.2 & 0.0 \\ 
  cbip\_80\_0.2 & 51.1 & 51.6 &  3.5 & 51.2 & 51.6 & 30.9 & 0.2 & 0.0 & 51.2 & 51.6 & 21.3 & 0.2 & 0.0 \\ 
  cbip\_80\_0.4 & 47.1 & 47.4 &  7.9 & 47.2 & 47.4 & 23.8 & 0.1 & 0.0 & 47.2 & 47.4 & 35.3 & 0.1 & 0.0 \\ 
  cbip\_80\_0.6 & 46.2 & 46.4 &  1.1 & 46.2 & 46.4 & 10.8 & 0.1 & 0.0 & 46.2 & 46.4 & 12.3 & 0.1 & 0.0 \\ 
  cbip\_80\_0.8 & 44.7 & 44.8 & 19.8 & 44.8 & 44.8 & 24.0 & 0.1 & 0.0 & 44.8 & 44.8 & 25.6 & 0.1 & 0.0 \\ 
   \hline
Mean & 39.8 & 40.0 & 8.8 & 39.9 & 40.0 & 25.2 & 0.2 & 0.0 & 39.9 & 40.0 & 25.5 & 0.2 & 0.0 \\
\hline
\end{tabular}
\end{table}


\begin{table}[ht]
\centering
\footnotesize
\captionsetup{font=small}
\caption{BRKGA results for the DIMACS instances}
\begin{tabular}{l|rrr|rrrrr|rrrrr}
  \hline
\multicolumn{1}{c|}{} & 
\multicolumn{3}{c|}{BRKGA} & 
\multicolumn{5}{c|}{BRKGA+R} & 
\multicolumn{5}{c}{BRKGA+R+LS} \\
instance & mean & max & ttb & mean & max & ttb & $diff_{m}$ & $diff_{x}$ & mean & max & ttb & $diff_{m}$ & $diff_{x}$ \\ 
  \hline
brock200\_2.clq &  44.2 &  45.0 & 145.4 &  45.3 &  48.0 & 282.9 & 2.4 & 6.7 &  45.5 &  49.0 & 325.2 & 2.8 & 8.9 \\ 
  c-fat200-1.clq &  18.0 &  18.0 &   0.2 &  18.0 &  18.0 &   0.2 & 0.0 & 0.0 &  18.0 &  18.0 &   0.3 & 0.0 & 0.0 \\ 
  c-fat200-2.clq &  35.0 &  35.0 &   1.4 &  35.0 &  35.0 &   1.1 & 0.0 & 0.0 &  35.0 &  35.0 &   2.1 & 0.0 & 0.0 \\ 
  c-fat200-5.clq &  86.8 &  87.0 &   2.6 &  86.8 &  87.0 &   2.3 & 0.0 & 0.0 &  86.7 &  87.0 &  31.7 & 0.1 & 0.0 \\ 
  c-fat500-1.clq &  21.0 &  21.0 &   4.1 &  21.0 &  21.0 &   3.3 & 0.0 & 0.0 &  21.0 &  21.0 &   3.9 & 0.0 & 0.0 \\ 
  c-fat500-2.clq &  39.0 &  39.0 &  39.7 &  39.0 &  39.0 &  30.2 & 0.0 & 0.0 &  39.0 &  39.0 &  31.6 & 0.0 & 0.0 \\ 
  C125.9.clq &  76.8 &  78.0 &  70.5 &  77.1 &  78.0 & 147.9 & 0.4 & 0.0 &  77.3 &  79.0 & 135.8 & 0.6 & 1.3 \\ 
  DSJC125.1.col &  12.6 &  13.0 &  29.4 &  13.0 &  13.0 &  20.0 & 3.2 & 0.0 &  13.0 &  13.0 &  19.6 & 3.2 & 0.0 \\ 
  DSJC125.5.col &  35.9 &  38.0 &  47.3 &  37.3 &  38.0 & 237.5 & 3.8 & 0.0 &  37.1 &  38.0 & 202.9 & 3.2 & 0.0 \\ 
  DSJC125.9.col &  76.5 &  78.0 &  58.5 &  76.7 &  78.0 & 127.9 & 0.2 & 0.0 &  76.8 &  78.0 & 160.9 & 0.4 & 0.0 \\ 
  DSJC250.1.col &  18.0 &  18.0 &  53.9 &  18.0 &  18.0 &  81.8 & 0.0 & 0.0 &  18.0 &  18.0 &  80.2 & 0.0 & 0.0 \\ 
  DSJR500.1.col &  20.0 &  20.0 &   7.1 &  20.0 &  20.0 &   7.4 & 0.1 & 0.0 &  20.0 &  20.0 &   8.2 & 0.1 & 0.0 \\ 
  fpsol2.i.2.col &  40.0 &  40.0 &  36.8 &  40.0 &  40.0 &  30.6 & 0.1 & 0.0 &  40.0 &  40.0 &  58.3 & 0.1 & 0.0 \\ 
  fpsol2.i.3.col &  40.0 &  40.0 &  48.6 &  40.0 &  40.0 &  46.1 & 0.0 & 0.0 &  40.0 &  40.0 &  68.7 & 0.0 & 0.0 \\ 
  hamming6-2.clq &  40.0 &  40.0 &   0.2 &  40.0 &  40.0 &   0.2 & 0.0 & 0.0 &  40.0 &  40.0 &   0.5 & 0.0 & 0.0 \\ 
  hamming6-4.clq &  14.0 &  15.0 &  57.4 &  14.1 &  16.0 &  77.0 & 1.0 & 6.7 &  14.2 &  15.0 & 112.8 & 1.9 & 0.0 \\ 
  hamming8-2.clq & 159.9 & 161.0 & 199.9 & 160.0 & 161.0 & 220.9 & 0.1 & 0.0 & 160.0 & 160.0 & 491.4 & 0.1 & 0.6 \\ 
  hamming8-4.clq &  38.2 &  39.0 &  80.5 &  38.3 &  39.0 & 131.0 & 0.2 & 0.0 &  38.5 &  42.0 & 118.6 & 0.7 & 7.7 \\ 
  johnson8-2-4.clq &  12.0 &  12.0 &   6.1 &  12.0 &  12.0 &   1.6 & 0.0 & 0.0 &  12.0 &  12.0 &   1.1 & 0.0 & 0.0 \\ 
  johnson8-4-4.clq &  29.2 &  31.0 & 116.7 &  30.1 &  31.0 & 252.1 & 3.1 & 0.0 &  30.0 &  31.0 & 219.0 & 2.7 & 0.0 \\ 
  keller4.clq &  45.5 &  48.0 & 140.4 &  46.5 &  51.0 & 287.5 & 2.2 & 6.2 &  47.2 &  50.0 & 363.5 & 3.7 & 4.2 \\ 
  le450\_15a.col &  31.3 &  32.0 & 157.5 &  31.5 &  32.0 & 234.0 & 0.7 & 0.0 &  31.5 &  32.0 & 258.0 & 0.7 & 0.0 \\ 
  le450\_15b.col &  31.8 &  32.0 & 167.9 &  32.1 &  33.0 & 239.6 & 1.0 & 3.1 &  32.1 &  33.0 & 248.3 & 0.9 & 3.1 \\ 
  le450\_25a.col &  43.3 &  44.0 & 135.9 &  43.6 &  44.0 & 199.3 & 0.7 & 0.0 &  43.8 &  44.0 & 245.1 & 1.2 & 0.0 \\ 
  le450\_25b.col &  42.1 &  43.0 & 124.1 &  42.3 &  44.0 & 167.8 & 0.5 & 2.3 &  42.6 &  44.0 & 201.9 & 1.1 & 2.3 \\ 
  le450\_5a.col &  18.0 &  19.0 & 119.4 &  18.0 &  19.0 & 130.2 & 0.1 & 0.0 &  18.0 &  19.0 & 135.0 & 0.1 & 0.0 \\ 
  le450\_5b.col &  18.0 &  18.0 & 112.1 &  18.0 &  18.0 & 105.0 & 0.1 & 0.0 &  18.0 &  18.0 &  89.6 & 0.0 & 0.0 \\ 
  le450\_5c.col &  22.1 &  23.0 & 158.2 &  22.3 &  23.0 & 221.4 & 0.8 & 0.0 &  22.2 &  23.0 & 210.8 & 0.7 & 0.0 \\ 
  le450\_5d.col &  21.9 &  22.0 & 172.0 &  22.1 &  23.0 & 168.7 & 0.5 & 4.5 &  22.0 &  23.0 & 178.2 & 0.5 & 4.5 \\ 
  MANN\_a9.clq &  21.0 &  21.0 &   0.0 &  21.0 &  21.0 &   0.0 & 0.0 & 0.0 &  21.0 &  21.0 &   0.1 & 0.0 & 0.0 \\ 
  mulsol.i.1.col &  52.0 &  52.0 &   4.4 &  52.0 &  52.0 &   3.7 & 0.0 & 0.0 &  52.0 &  52.0 &   9.6 & 0.0 & 0.0 \\ 
  mulsol.i.2.col &  33.5 &  34.0 &  69.0 &  33.9 &  34.0 & 188.8 & 1.0 & 0.0 &  34.0 &  34.0 & 214.3 & 1.3 & 0.0 \\ 
  mulsol.i.3.col &  33.6 &  34.0 &  41.6 &  34.0 &  34.0 & 133.2 & 1.2 & 0.0 &  33.9 &  34.0 & 164.4 & 1.0 & 0.0 \\ 
  mulsol.i.4.col &  33.5 &  34.0 &  65.4 &  34.0 &  34.0 & 179.7 & 1.4 & 0.0 &  34.0 &  34.0 & 184.5 & 1.4 & 0.0 \\ 
  mulsol.i.5.col &  34.0 &  34.0 &   0.4 &  34.0 &  34.0 &   0.3 & 0.0 & 0.0 &  34.0 &  34.0 &   3.3 & 0.0 & 0.0 \\ 
  R125.1.col &   7.0 &   7.0 &   0.0 &   7.0 &   7.0 &   0.0 & 0.0 & 0.0 &   7.0 &   7.0 &   0.0 & 0.0 & 0.0 \\ 
  R125.1c.col &  62.0 &  62.0 &   0.8 &  62.0 &  62.0 &   0.7 & 0.0 & 0.0 &  62.0 &  62.0 &   9.3 & 0.0 & 0.0 \\ 
  R125.5.col &  63.8 &  65.0 &  41.6 &  64.4 &  65.0 & 147.0 & 0.9 & 0.0 &  64.4 &  65.0 & 170.3 & 0.9 & 0.0 \\ 
  R250.1.col &  12.0 &  12.0 &  16.5 &  12.0 &  12.0 &  11.6 & 0.0 & 0.0 &  12.0 &  12.0 &  10.0 & 0.0 & 0.0 \\ 
  zeroin.i.1.col &  52.9 &  53.0 &  88.0 &  53.0 &  53.0 & 105.8 & 0.2 & 0.0 &  53.0 &  53.0 & 143.8 & 0.2 & 0.0 \\ 
  zeroin.i.2.col &  35.1 &  37.0 &  55.0 &  35.5 &  37.0 & 121.8 & 1.3 & 0.0 &  35.2 &  37.0 &  73.8 & 0.5 & 0.0 \\ 
  zeroin.i.3.col &  35.0 &  37.0 &  45.8 &  35.2 &  37.0 &  58.6 & 0.4 & 0.0 &  35.2 &  37.0 & 101.8 & 0.6 & 0.0 \\
   \hline
Mean & 38.2 & 38.8 & 64.9 & 38.4 & 39.0 & 104.9 & 0.6 & 0.7 & 38.5 & 39.1 & 121.1 & 0.7 & 0.7 \\
\hline
\end{tabular}
\end{table}
\end{comment}

==> 97_test_appendice_image.tex <==
\section{Somente para testar e deixar salvo o formato geral}
\MateusF{Não estão padronizadas ainda não}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/c_barplot_betterorequalmax.pdf}
    \caption{Caption}
    %\label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/c_boxplot_diff_maxall_0.pdf}
    \caption{Caption}
    %\label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/c_boxplot_diff_maxall_dimacs.pdf}
    \caption{Caption}
    %\label{fig:enter-label}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.5\linewidth]{images/c_boxplot_diff_maxall_small.pdf}
    \caption{Caption}
    %\label{fig:enter-label}
\end{figure}

==> 98_IG.tex <==
The Algorithm \ref{alg:decoder_con_grundy_ig} describes a local search using iterated greedy and the decoder for the solution reconstruction step. The line \ref{deccig:init-aChromosome} initiates an artificial chromosome with size $O(|V|)$ that will be used in the reconstruction and will replace the chromosome having the values referring to the new order that wants to be created. Line \ref{deccig:auxCont} creates a variable that will assist in creating the artificial chromosome keys. Lines \ref{deccig:rcl}-\ref{deccig:pl} creates a list of restricted candidates based on the keys of the second half of the chromosome with a maximum size of $maxsize$. After that, a percentage of vertices present in $RCL$ are randomly chosen and inserted into $filteredList$ accordingly, maintaining the relative order between them in the original order of the solution $S$. These elements are the ones that will be removed. Finally, the list $PL$ is created which has the other vertices also maintaining the relative order between them and these are the ones that have the highest priority in the reconstruction. Lines \ref{deccig:iPL}-\ref{deccig:fFL} are responsible for setting the value of the keys of each vertex according to the new priority that will be given to them. Line \ref{deccig:reconstruct} calls the decoder to reconstruct the solution, and in lines \ref{deccig:compare}-\ref{deccig:call} checks if the new solution $S'$ is better than the previous one $S$ and if so, the local search continues calling the function again passing the new solution $S'$. Otherwise, it ends the local search returning the last best solution found.

\begin{algorithm}[!ht]
\caption {LocalSearch-IG ($G$, $S$, $c$, $maxsize$, $\alpha$) }
\label{alg:decoder_con_grundy_ig}
    $aChromosome \leftarrow \{0,\ldots, 0\}$\; \label{deccig:init-aChromosome}
    $i \leftarrow 0$ \; \label{deccig:auxCont}
    $RCL \leftarrow$ SelectVertexToRemove($S$, $c$, $maxsize$)\; \label{deccig:rcl}
    $filteredList \leftarrow$ SelectVertexToRemoveInOrder($S$, $RCL$, , $\alpha*maxsize$)\; \label{deccig:filtered}
    $PL \leftarrow$ PriorityVertexInOrder($S$, $filteredList$)\; \label{deccig:pl}
    \ForEach{$v \in PL$}{ \label{deccig:iPL}
       $aChromosome[v] \leftarrow |G.V|-i$\;
       $i \leftarrow i+1$\;
    } \label{deccig:fPL}
    \ForEach{$v \in filteredList$}{ \label{deccig:iFL}
       $aChromosome[v] \leftarrow i*(-1)$\;
       $i \leftarrow i+1$\;
    }\label{deccig:fFL}
    $S' \leftarrow $ Decoder-connected($G$, $aChromosome$)\; \label{deccig:reconstruct}
    \If{$S'.fitness > S.fitness$}{ \label{deccig:compare}
        \Return Decoder-CG-IG($G$, $S'$, $c$, $maxsize$, , $\alpha$)\;\label{deccig:call}
    }
    \Return $S$\; \label{deccig:return}
\end{algorithm}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
